Low-Power IoT Communication Security: On the Performance of DTLS and TLS 1.3

Similarly to elsewhere on the Internet, practical security in the Internet of Things (IoT) is achieved by combining an array of mechanisms, at work at all layers of the protocol stack, in system software, and in hardware. Standard protocols such as Datagram Transport Layer Security (DTLS 1.2) and Transport Layer Security (TLS 1.2) are often recommended to secure communications to/from IoT devices. Recently, the TLS 1.3 standard was released and DTLS 1.3 is in the final stages of standardization. In this paper, we give an overview of version 1.3 of these protocols, and we provide the first experimental comparative performance analysis of different implementations and various configurations of these protocols, on real IoT devices based on low-power microcontrollers. We show how different implementations lead to different compromises. We measure and compare bytes-over-the-air, memory footprint, and energy consumption. We show that, when DTLS/TLS 1.3 requires more resources than DTLS/TLS 1.2, this additional overhead is quite reasonable. We also observe that, in some configurations, DTLS/TLS 1.3 actually decreases overhead and resource consumption. All in all, our study indicates that there is still room to optimize the existing implementations of these protocols.

==> Text/discussion.tex <==
\section{Towards Smaller Footprint Communication Security}\label{sec:future}

Recent work has started to focus on minimizing communication security footprint.
\ \\
\paragraph*{Compacting TLS}
For instance, cTLS (Compact TLS 1.3~\cite{I-D.draft-rescorla-tls-ctls})
proposes a configuration of TLS 1.3 which sacrifices backwards compability
for significant savings in over-the-wire size.
This effort leverages both aggressive use of a more compact encoding, and the use of default values for TLS configurations.
\ \\
\paragraph*{Object Security}
Aside of TLS and DTLS, alternative communication security solutions have also emerged.
The most prominent alternatives targeting IoT are based on COSE~\cite{RFC8152} and OSCORE~\cite{RFC8613},
which aim at securing transferred data higher up in the protocol stack, i.e. at the application layer and at the CoAP layer, respectively.

{\bf CBOR Object Signing and Encryption (COSE)}~\cite{RFC8152} is a signing and encryption scheme which is conceptually similar to JavaScript Object Signing and Encryption (JOSE).
COSE can be used in "standalone" fashion to protect data transmitted over the network. 
%COSE can be seen as a set of building blocks that applications use in the way they find useful (with an eye on code size). 
COSE offers digital signatures, counter signatures, Message Authentication Codes (MACs), encryption, and rudimentary key distribution methods. 
COSE is a good fit for securing "one-shot" messages or objects in transit or at rest somewhere in the network. For instance, a COSE usecase is protecting a firmware update binary (or more precisely, for signing metadata about the firmware and, optionally, encrypting the firmware image~\cite{DBLP:journals/access/ZandbergSPTB19}). 
Another COSE usecase is protecting access tokens used with the ACE-OAuth framework. 


% OSCORE
{\bf Object Security for Constrained RESTful Environments}~\cite{RFC8613} reuses COSE to protect CoAP messages, or more precisely some CoAP headers and the CoAP payload. 
It does not protect the entire CoAP message because CoAP proxies have to inspect part of the message. 
%The authors of CoAP defined the interaction between CoAP and DTLS slightly differently to how HTTP did. 
%In CoAP, DTLS is terminated at the proxy, while in HTTP a TLS exchange is transparently passed through (unless it is a reverse proxy). 
%In context of OSCORE, these proxies can also be special CoAP-to-HTTP proxies as long as they do not change the nature of the REST API interaction. 

Since OSCORE does not offer key management itself, it has to rely on a separate key management protocol. 
The ACE-OAuth framework~\cite{I-D.ietf-ace-oauth-authz} can be reused to facilitate such key management. 
Other key management protocols currently investigated in the IETF are Ephemeral Diffie-Hellman over COSE (EDHOC) and Application Layer TLS (ATLS)~\cite{I-D.friel-tls-atls}. 
Both, EDHOC and ATLS, allow the establishment of an OSCORE security context. 
EDHOC rebuilds a handshake protocol based on COSE while ATLS uses TLS and DTLS at the application layer. 
\ \\
\paragraph*{Other approaches}
Approaches to secure communication also include a variety of other mechanisms. For instance, standards such as IPsec with the key management protocol IKEv2, or the Host Identity Protocol (HIP) could be used. In this paper however, we do not further consider these approaches (or other non-standard schemes, for that matter) because from our perspective, the community working on low-end IoT currently tends to polarize on developing and comparing the alternative OSCORE with EDHOC versus TLS/DTLS, or ATLS over CoAP.
% TBD: Discuss ongoing standardization work around cTLS and other extensions we have not looked at? 

\subsection{Perspectives}
Our observation is that optimal performance of TLS / DTLS 1.3 on microcontrollers is still to be determined.
In particular, comparing this performance to that of solutions based on OSCORE and EDHOC is future work.

On one hand, work aiming to minimize TLS/DTLS 1.3 footprint is currently in early stages of development in the TLS working group and needs futher evaluation down the line, in order to gauge its full potential.
Recent work has started to focus on minimizing communication security footprint.
For instance, cTLS (Compact TLS 1.3~\cite{I-D.draft-rescorla-tls-ctls})
proposes a configuration of TLS 1.3 which sacrifices backwards compability
for significant savings in over-the-wire size.
This effort leverages both aggressive use of a more compact encoding, and the use of default values for TLS configurations.

On the other hand, EDHOC specification is also work-in-progress. Maturation of this solution is expected to happen next within the newly formed IETF working group LAKE~\cite{LAKE-wg}.

Furthermore, on top of the metrics we measured experimentally in this paper it would be useful to extend these studies to the above-mentioned protocols. 

% While standardized benchmarks, even based on a synthetic TLS 1.2 handshake, exist with the work by the Embedded Microprocessor Benchmark Consortium (EEMBC) on SecureMark-TLS~\cite{SecureMark-TLS} very few reseachers have scores on this standard for off-the-shelf, low-end microcontrollers. 
\ \\

==> Text/evaluation.tex <==
\subsection{Experimental Results}
\label{sec:evaluation}
The quantitative analysis is split into two parts. First, we analyze the performance of TLS/DTLS 1.2 to have a metric for comparison.  Second, we evaluate the performance of the 1.3 counterparts.

Table~\ref{tab:flash} gives an overview of the total flash memory requirements of the different profiles (in kB). Subsequently, we investigate the contributions of the different components in more detail. The profiles are described in Section~\ref{sec:test-setup}.

\begin{center}
\begin{table*}[ht]
        \begin{tabular}{l|ccccc}
   \toprule
              Component & PSK (128 bit) & PSK (128 + 256 bit) & ECDSA-ECDSA (128 bit) & ECDSA-ECDSA (128+256 bit) & Full\\
   \midrule
          TLS 1.2 	&  20 & 24 & 57 & 63 & 65 \\
          TLS 1.3    &  22 & 27 & 63 & 65 & 68 \\
          DTLS 1.2 	&  24 & 29 & 61 & 69 & 76 \\
          DTLS 1.3  &  27 & 32 & 63 & 69 & 74 \\
   \bottomrule
  \end{tabular}
  \caption{Flash requirements (in kB) per profile, on a Cortex-M4 microcontroller.}
  \label{tab:flash}
\end{table*}
\end{center}

Table~\ref{tab:flash-cid} shows the difference between an implementation with and without CID support. As it can be seen, enabling CID support provides a number of over-the-wire and performance benefits without almost any impact on the flash size. The stack utilization is also not impacted by this extension. For a client-side DTLS implementation it therefore makes a lot of sense to enable the use of the CID feature. 
 
\begin{center}
\begin{table*}[ht]
        \begin{tabular}{l|cc}
   \toprule
              Component & without CID & with CID \\
   \midrule
          DTLS 1.2 PSK (128-bit)	&  24,972 &  25,796 \\
          DTLS 1.3 PSK (128-bit)  &  27,520 &  28,084 \\
   \bottomrule
  \end{tabular}
  \caption{Flash requirements (in Bytes), on a Cortex-M4 microcontroller.}
  \label{tab:flash-cid}
\end{table*}
\end{center}


Figure~\ref{fig:tls13-psk-128} breaks down the realtive flash memory requirements per component, for TLS 1.3 PSK with AES-128-CCM. Four major components are distinguished in this measurement along with the relevant Mbed TLS source file list for that component. Note that the code size needed for symmetric crypto is almost as large as the code size for the TLS protocol itself. 
\begin{description}
\item[TLS protocol:] This code includes the client-side of the TLS protocol (ssl\_cli.c) and code that is shared between the client and the server-side found in ssl\_tls.c. Additionally, there is code for managing ciphersuites (ssl\_ciphersuites.c).
\item[Symmetric Crypto:] This code includes SHA256, AES, CCM, and the wrapper functions for more convenient use of cryptographic primitives (sha256.c, ccm.c, cipher, cipher\_wrap, and md\_wrap, aes.c).
\item [Random Number Generation (RNG):] The code uses the Counter Mode Deterministic Random Byte Generator that was standardized by NISTentropy (ctr\_drbg.c, entropy.c and entropy\_poll.c).
\item [HKDF:] The HKDF functions specified in RFC 5869 (hkdf.c) as well as the TLS 1.3-specific use of it (hkdf-tls.c)
\end{description}

\begin{figure}[!t]
\centering
\includegraphics[width=6cm]{figures/tls13-psk-128}
\caption{Relative sizes of Flash memory per component, for TLS 1.3 PSK with AES-128-CCM.}
\label{fig:tls13-psk-128}
\end{figure}

Figure~\ref{fig:tls13-ecdsa-128} shows the realtive flash memory requirements per component for TLS 1.3 ECDSA-ECDHE (P2561) with AES-128-CCM. In addition to code size for the TLS 1.3 PSK shown in Figure~\ref{fig:tls13-psk-128} components for public key cryptography have to be taken into account. While the code size for the TLS library increased from 9.2 kB to 11.2 kB the bulk of the added code can be attributed to asymmetric crypto (16.7 kB) and X.509-related functions (10.5 kB).
\begin{description}
\item[Asymmetric Crypto:] This code includes the bignum library (bignum.c) as well as the functionality needed for the offering ECC, ECDSA, ECDHE (ecp\_curves.c, ecdsa.c, ecdh.c, and ecp.c).
\item[X509-related Functions:] This code includes ASN1 libraries (asn1write.c, and asn1parse.c), public key processing functions (pkparse.c) and various support functions (base64.c, pk.c, pk\_wrap.c, pem.c, and oid.c).
\end{description}

\begin{figure}[!t]
\centering
\includegraphics[width=6cm]{figures/tls13-ecdsa-128}
\caption{Relative sizes of Flash memory per component, for TLS 1.3 ECDSA-ECDHE (P2561) with AES-128-CCM.}
\label{fig:tls13-ecdsa-128}
\end{figure}

Table~\ref{tab:flash-values} shows the absolute values of the Flash memory size of the different components for the two profiles profile (in Bytes). Note that the PSK profile does not include support for an ECDHE exchange; this would require support for asymmetric crypto and thereby reducing the benefits of a PSK-based profile. A better alternative would be to switch from pre-shared secrets to the use of raw public keys in this case because the support for X.509 is not required. The use of raw public keys is unfortunately not included in the mainstream version of the Mbed TLS codebase and the experimental code available still requires the use of the X.509 libraries due to a coding design decision. For this reason the functionality has not been tested in this paper. 

\begin{table*}[ht]
        \begin{tabular}{l | c c c c c c}
   \toprule
             Profile & TLS & Sym. Crypto & RNG & HKDF & Asym. Crypto & X.509\\
   \midrule
          TLS 1.3 PSK with AES-128-CCM    &   9511 &  9335 & 1424 &  1812 & N/A &  N/A \\
          TLS 1.3 ECDSA-ECDHE (P2561) with AES-128-CCM &  11497 & 9335 & 1424 &  1812 & 17168 & 10842 \\
          \bottomrule
  \end{tabular}
  \caption{Flash requirements (in Bytes) for components, per profile, on a Cortex-M4 microcontroller.%
    \label{tab:flash-values}}
\end{table*}

Table \ref{tab:RAM} shows the RAM memory requirements (stack) for TLS and DTLS, compared for different configurations, for versions 1.2 and 1.3 of the protocols. We observe that for all profiles, and all versions, RAM requirements (stack) remains roughly the same around 8.8kB which is bearable on most modern microcontrollers.

Finally, Figure~\ref{fig:tls-over-the-wire} shows the over-the-wire overhead of the different profiles, in Bytes. We observe that, indeed, as expected per the changes we observed on a protocol level in Section~\ref{sec:overview}, less bits are transmitted over the network.

%\begin{center}
\begin{table*}[ht]
        \begin{tabular}{l|ccccc}
   \toprule
              Component & PSK (128 bit) & PSK (128 + 256 bit) & ECDSA-ECDSA (128 bit) & ECDSA-ECDSA (128+256 bit) & Full\\
   \midrule
          TLS 1.2  & 8828 & 8816 & 8848 & 8848 & 8848 \\
          TLS 1.3  & 8792 & 8804 & 8840 & 8840 & 8840 \\
          DTLS 1.2 & 8824 & 8828 & 8836 & 8848 & 8872 \\
          DTLS 1.3 & 8812 & 8812 & 8836 & 8840 & 8836 \\
   \bottomrule
  \end{tabular}
  \caption{RAM requirements (in Bytes), per profile, on a Cortex-M4 microcontroller.}
  \label{tab:RAM}
\end{table*}
%\end{center}


\begin{figure*}[!t]
\centering
\includegraphics[width=\textwidth,height=4.5cm]{figures/tls-over-the-wire}
\caption{Over-the-wire overhead (in Bytes).}
\label{fig:tls-over-the-wire}
\end{figure*}

\subsection{Summary \& Observations}
A TLS/DTLS stack consists of a number of components and the code size is heavily influenced by the size of the underlying crypto primitives being used. The TLS/DTLS protocol implementation itself contributes less than half of the code size for a PSK-based implementation and less than 25\% of the code size for a public key-based implementation. This has to be taken into account when aiming for code size optimizations, particularly because various crypto implementations are available to developers and algorithms other than the NIST P-256-based ECC curves can be selected. 

A PSK-based implementation of TLS/DTLS is, of course, substantially smaller than a corresponding public key based implementation. The difference between an implementation that offers 128-bits and another one that offers 128-bits and 256-bits is small and typically around 5 kB for the additional SHA516 library. The difference between a public key based profile and a full implementation is fairly small, again around 5 kB. The extra code size for the extra features, such as 0-RTT, backwards compability mode, ticket extensions, looks worth the extra additional codesize.  

To our surprise, the difference of RAM utilization between version 1.2 and 1.3 is largely irrelevant. The smaller message size for the public key-based authentication mode is a positive development even though the handshake messages themselves will be less frequently exchanged in an IoT environment considering the availability of the CID extension, which we highly recommend using because it allows to maintain an established session for weeks or even months. 
\ \\

==> Text/introduction-short.tex <==

\section{Introduction}\label{sec:introduction}

As the Internet of Things (IoT) deployment unfolds, the list of attacks against IoT devices gets longer.
To address the security concerns,
governmental institutions, industry groups, and researchers have been publishing recommendations and guidelines for securing IoT devices. 
Examples include the `Baseline Security Recommendations for IoT'~\cite{ENISA} published by the European Union Agency for Cybersecurity (ENISA) and the `Core Cybersecurity Feature Baseline for Securable IoT Devices: A Starting Point for IoT Device Manufacturers'~\cite{NIST} published by 
the National Institute of Standards and Technology (NIST).
Renowned security expert Bruce Schneier~\cite{Schneier} published a long list of available guidelines and it is immediately clear that there is no shortage on advice for IoT manufacturers and embedded developers.

While these sets of guidelines vary in the level of detail, they all ask for communication security to be integrated into IoT devices. 
Over the years, Transport Layer Security (TLS) has become the most widely used (and the most carefully scrutinized) approach to secure data in transit over the Internet.
To no surprise, some IoT security guidelines actually mandate the use of TLS to provide end-to-end communication integrity, confidentiality and authenticity.
Version 1.2 of TLS~\cite{RFC7925} has so far been the recommended standard for securing protocols operating over TCP, along with its UDP-based variant Datagram Transport Layer Security (DTLS).


Recently, TLS 1.3~\cite{RFC8446} was published, and DTLS 1.3 is in the final stages of standardization.
A reasonable question is thus: How appropriate is TLS 1.3 for IoT?
In particular, we focus here on resource-constrained IoT devices, such as described in RFC 7228~\cite{RFC7228}. These devices are based on microcontrollers -- for instance Arm Cortex M-based  microcontrollers -- on which run real-time operating systems, such as FreeRTOS, RIOT, Micrium's $\mu$C/OS, Mbed OS, among others~\cite{hahm2016surveyOS}. 
Compared to computers that run full-blown operating systems, such as Linux, constrained IoT devices use a fraction of the power and are equipped with RAM and Flash sizes in the kilobyte range.

{\bf Related work --} 
There is so far surprisingly little work evaluating DTLS/TLS 1.3 on IoT hardware.
The only prior work we know of is \cite{bossi2016tls13}, which evaluates a preliminary draft version of TLS 1.3 on STM32-based microcontrollers.
Compared to \cite{bossi2016tls13}, our paper analyzes the final TLS 1.3 standard, as well as the latest version of DTLS 1.3.

Open source implementation of DTLS 1.3 we know of so far are limited to a partial implementation in Go ~\cite{Mint-DTLS} and a prototype in Mozilla NSS~\cite{NSS}, neither of which fit in an embedded network stack applicable to microcontrollers.
%To the best of our knowledge, this paper presents the first experimental study evaluating and comparing DTLS/TLS 1.2 with DTLS/TLS 1.3, on low-power microcontrollers.

%{\bf Paper contributions --}
The main contributions of this paper are the following:
\begin{itemize}
%\item we provide a comparative overview of DTLS/TLS 1.3 and 1.2 protocol specifications;
\item we provide the first open source implementation of the DTLS 1.3 protocol targeting small embedded systems;
\item we conduct experiments on IoT microcontrollers, comparing the performance of different configuration and multiple implementations of DTLS/TLS 1.3 and 1.2;
\item we measure and compare the footprint of secure communication solutions in terms of bytes over-the-air, RAM and Flash memory requirements, energy consumption;
\item we overview next steps and optimization potential towards lower footprint with IoT communication security at the transport layer and above.
\end{itemize}

\iffalse
{\bf Paper organization --} 
This paper is organized as follows:
In Section~\ref{sec:background}-\ref{sec:overview} provides necessary background on TLS, DTLS and overviews protocol differences between 1.3 and 1.2 versions.
In Section~\ref{sec:test-setup} we describe our experimental test setup. 
In Section~\ref{sec:evaluation} we present the results of our comparative performance evaluation, based on memory, traffic overhead, and energy measurements. 
Then, in Section~\ref{sec:future} we discuss perspectives, before we conclude. 
\ \\
\fi



==> Text/related-work.tex <==
\section{Related Work}\label{sec:related-work}

In addition to TLS/DTLS, the IETF offers other communication security solutions as well, namely 
\begin{itemize}
\item Object Security for Constrained RESTful Environments (OSCORE ~\cite{RFC8613}),
\item IPsec with the key management protocol IKEv2, and 
\item the Host Identity Protocol (HIP). 
\end{itemize}

The development of OSCORE initially started as an application layer security solution protecting CoAP messages traversing also CoAP proxies. Later, it was extended to work also when CoAP traffic is mapped to HTTP because end-to-end communication in IoT deployments rarely uses CoAP alone.

OSCORE reuses CBOR Object Signing and Encryption (COSE)~\cite{RFC8152} to protect CoAP messages, or more precisely some CoAP headers and the CoAP payload. It cannot protect the entire CoAP message because CoAP proxies have to inspect part of the message. The authors of CoAP defined the interaction between CoAP and DTLS slightly differently to how HTTP did. In CoAP, DTLS is terminated at the proxy, while in HTTP a TLS exchange is transparently passed through (unless it is a reverse proxy). In context of OSCORE, these proxies can also be special CoAP-to-HTTP proxies as long as they do not change the nature of the REST API interaction. 

Since OSCORE does not offer key management itself, it has to rely on a separate key management protocol. The ACE-OAuth framework~\cite{I-D.ietf-ace-oauth-authz} can be reused to facilitate such key management. Other key management protocols currently investigated in the IETF are Ephemeral Diffie-Hellman over COSE (EDHOC) and Application Layer TLS (ATLS)~\cite{I-D.friel-tls-atls}. EDHOC is a competitor to TLS/DTLS and ATLS. Both, EDHOC and ATLS, allow the establishment of an OSCORE security context. EDHOC rebuilds a handshake protocol based on COSE while ATLS uses TLS and DTLS at the application layer. 

In this section we focus on security technologies that are tailored toward one-shot payloads. For example, consider a scenario where firmware images are distributed by the device management server and must be secured end-to-end, from the developer to the IoT device. Since the firmware image may be stored on servers for an extended period of time and must be self-contained, a different security mechanism, such as, is more appropriate, and we cover it next. 

COSE, a recently developed signing and encryption scheme, which is conceptually similar to JavaScript Object Signing and Encryption (JOSE),  alone can be used to protect data. COSE can be seen as a set of building blocks that applications use in the way they find useful (with an eye on code size). COSE offers digital signatures, counter signatures, Message Authentication Codes (MACs), encryption, and rudimentary key distribution methods. 

Most security services are offered in two versions, depending on whether one or multiple entities create or receive them. For example, the COSE\_Sign1 signature structure is used when only one signature will be placed on a message, whereas COSE\_Sign allows for one or more signatures to be applied. COSE\_Sign1 and COSE\_Sign are different structures and cannot be converted from one to the other. 

Since CBOR is a good fit for securing data when the goal is to protect one-shot messages or objects in transit and also at rest, the use of COSE is one option for protecting firmware updates, or more precisely, for signing metadata about the firmware and, optionally, encrypting the firmware image. COSE can also protect access tokens used with the ACE-OAuth framework. 


TBD: Something about IPsec and maybe about HIP



==> Text/test-setup-short.tex <==
\section{Experimental Setup}
\label{sec:test-setup}
The full details of our setup (compiler, toolchain, software versions, ciphersuites...) are available in the report~\cite{arxiv-2020}.
Our experiments were carried out on a variety of IoT devices from Nordic, Keil, and STMicro, based on various common Arm Cortex-M microcontrollers, and typical low-power radios.
To perform energy measurements, we primarily used the {\bf Nordic nRF6707} power profiling kit.

We provide an implementation of DTLS 1.3 targeting low-power microcontrollers, the open source of which is published at~\cite{Hannes-DTLS13}.
We comparatively evaluate this base with different implementations (mbedTLS 2.16, and WolfSSL 4.4.0) of various configurations of DTLS and TLS protocols, versions 1.2 and 1.3.

For our setup, we used RIOT~\cite{2018-RIOT} as the real-time operating system in version 2019.10, which includes networking middleware.
Our setup uses two RIOT nodes communicating via a 6LoWPAN/CoAP protocol stack, including support for different DTLS/TLS libraries and configurations.
We wrote an application to test the different configurations and the code is published at~\cite{Gabriele-RIOT-branch} for reproduceability. Our application uses TLS and DTLS on top of CoAP, as specified in~\cite{I-D.friel-tls-atls}.

Our measurements capture the entire protocol exchange, including RTOS handling, network communication, processing by the networking stack, as well as the entire TLS/DTLS handshake. We start the measurement when the first packet is sent out to initiate the TLS/DTLS handshake and stop it when we close the TLS/DTLS handshake.

\paragraph*{Metrics}
To comparatively evaluate the protocols and their implementations, we measure the required 
(i) stack and heap size,
(ii) code size,
(iii) over-the-wire network traffic overhead,
and (iv) energy consumption.

\iffalse
While the absolute numbers are important they ignore the flexibility of embedded TLS stacks whereby the crypto algorithms can be optimized, or replaced by another software implementation. In some cases, depending on the capability of the hardware, the TLS stack can also make use of crypto accelerators in hardware. Note that we did not utilize hardware crypto acceleration provided by the nRF52840-DK. Prior work, such as~\cite{DBLP:journals/access/ZandbergSPTB19}, investigates different embedded crypto libraries and noted the tradeoffs made by different implementations. Hence, we have included tests with different TLS/DTLS implementations.
\fi

